Fast Context-Annotated Classification of Different Types of Web Service Descriptions

In the recent rapid growth of web services, IoT, and cloud computing, many web services and APIs appeared on the web. With the failure of global UDDI registries, different service repositories started to appear, trying to list and categorize various types of web services for client applications' discover and use. In order to increase the effectiveness and speed up the task of finding compatible Web Services in the brokerage when performing service composition or suggesting Web Services to the requests, high-level functionality of the service needs to be determined. Due to the lack of structured support for specifying such functionality, classification of services into a set of abstract categories is necessary. We employ a wide range of Machine Learning and Signal Processing algorithms and techniques in order to find the highest precision achievable in the scope of this article for the fast classification of three type of service descriptions: WSDL, REST, and WADL. In addition, we complement our approach by showing the importance and effect of contextual information on the classification of the service descriptions and show that it improves the accuracy in 5 different categories of services.

==> setup.tex <==
\usepackage[latin1]{inputenc}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{latexsym}
\usepackage{makeidx}
\usepackage{style/cuthesis}
\usepackage{style/named}
\usepackage{url}
\usepackage{listings}
\usepackage{amsthm}
%\usepackage{empheq}
\usepackage{caption}
\usepackage{fullpage}

\usepackage{array}
\usepackage{multirow}
\usepackage{setspace}
	\usepackage[%
		lmargin=1.5in,
		rmargin=1.0in,
		tmargin=1.0in,
		bmargin=1.0in,
		%includefoot
		]{geometry}
\usepackage{fancyhdr}
\usepackage[nottoc, notlof, notlot]{tocbibind}
\usepackage{minitoc}
\usepackage[intoc]{nomencl}
\setcounter{minitocdepth}{2}
\mtcindent=15pt
\hyphenpenalty 5000
\tolerance=10000

\usepackage{tabu}
\usepackage{longtable}

\usepackage{xparse}
% It should be loaded after all other packages
\usepackage[colorlinks,linkcolor=blue,urlcolor=blue,citecolor=blue]{hyperref}
\usepackage{listings}
\usepackage{color}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

\usepackage{algorithm}
%\usepackage{algpseudocode}
\usepackage{algorithmic}
%\usepackage{algorithm2e}

% Common commands
%
\input{common/commands}

\lstdefinestyle{codeStyle}{
    captionpos=b,%
    showstringspaces=false,%
    showspaces=false,
    frame=single,  %use this to have a box around the code
    %frame=htb, framerule=1pt, %Use this to have only top and bottom frames
    extendedchars=true,%
%    basicstyle=\tiny\tt, %use this for the smallest characters
    basicstyle=\scriptsize\tt, %use this for small, but not that small characters
    %basicstyle=\footnotesize\tt, %use this for normal, yet smaller characters
    linewidth=1\linewidth,%
%    language=[ANSI]C,%
    language=Java,%
    breaklines=true,
    float=phtb,  %change this to change where the floats end
%------------ Uncomment to make more compact
%    aboveskip=6pt,
%    belowskip=0pt,
%    abovecaptionskip=0pt,
%    belowcaptionskip=0pt
}

% Number all sections, but include only section and subsections in the ToC.
%\setcounter{secnumdepth}{4}
%\setcounter{tocdepth}{4}
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%
% Top heading
%
%	\begin{figure}
%		\includegraphics[width=20pt]{gipsystar}
%	\end{figure}
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{20}
\setcounter{dbltopnumber}{9}

 
